Scalable Stochastic Parametric Verification with Stochastic Variational Smoothed Model Checking

Parametric verification of linear temporal properties for stochastic models can be expressed as computing the satisfaction probability of a certain property as a function of the parameters of the model. Smoothed model checking (smMC) aims at inferring the satisfaction function over the entire parameter space from a limited set of observations obtained via simulation. As observations are costly and noisy, smMC is framed as a Bayesian inference problem so that the estimates have an additional quantification of the uncertainty. In smMC the authors use Gaussian Processes (GP), inferred by means of the Expectation Propagation algorithm. This approach provides accurate reconstructions with statistically sound quantification of the uncertainty. However, it inherits the well-known scalability issues of GP. In this paper, we exploit recent advances in probabilistic machine learning to push this limitation forward, making Bayesian inference of smMC scalable to larger datasets and enabling its application to models with high dimensional parameter spaces. We propose Stochastic Variational Smoothed Model Checking (SV-smMC), a solution that exploits stochastic variational inference (SVI) to approximate the posterior distribution of the smMC problem. The strength and flexibility of SVI make SV-smMC applicable to two alternative probabilistic models: Gaussian Processes (GP) and Bayesian Neural Networks (BNN). The core ingredient of SVI is a stochastic gradient-based optimization that makes inference easily parallelizable and that enables GPU acceleration. In this paper, we compare the performances of smMC against those of SV-smMC by looking at the scalability, the computational efficiency and the accuracy of the reconstructed satisfaction function.

==> sections/inference.tex <==
\section{Stochastic Variational Smoothed Model Checking}\label{sec:sv-smc}

The goal of Stochastic Variational Smoothed Model Checking (SV-smMC) is to efficiently infer an accurate probabilistic estimate of the unknown satisfaction function $f_\varphi:\Theta\to [0,1]$. In order to do so, we define a function $f:\Theta \to [0,1]$ that should behave as similarly as possible to $f_\varphi$.
The main ingredients of a Bayesian approach to the problem stated above are the following:
\begin{enumerate}

    \item Choose a \emph{prior} distribution, $p(f)$, over a suitable function space encapsulating the beliefs about function $f$ prior to any observations being taken.
    \item Determine the functional form of observation process by defining a suitable \emph{likelihood function} that effectively models how the  observations depend on the uncertain parameter $\theta$. Our observation process can be modeled by a binomial over $M_t$ trials with parameter $f_\varphi (\theta)$. Given the nature of our training set, defined in~\eqref{eq:train_dataset}, we define the probabilistic likelihood as 
    $$p(D_t| f) = \prod_{i=1}^{N_t} Binomial(L_i\mid M_t, f(\theta_i)).$$
    
    \item Leverage Bayes' theorem to define the \emph{posterior} distribution over functions given the observations
    $$
    p(f| D_t) = \frac{p(D_t| g)p(f)}{p(D_t)}.
    $$
    Computing $p(D_t) = \int p(D_t| f) p(f) df$ is almost always computationally intractable for non-conjugate prior-likelihood distributions. Therefore, we need algorithms to accurately approximate such posterior distribution.
    
    \item Evaluate statistics of such posterior at points $\theta_*$ and obtain the desired estimate of the satisfaction probability together with the respective confidence interval.
    
\end{enumerate}
SV-smMC leverages stochastic variational inference to efficiently compute the approximate posterior distribution $p(f|D_t)$ so that smMC inference scales well to large dataset $D_t$. In particular, SV-smMC proposes two alternative probabilistic models to define distributions over function $f$. The first one is based on Gaussian Processes (GP), whereas the second one is based on Bayesian Neural Networks (BNN).

\subsection{Gaussian Processes}\label{subsec:gp-smc}
A \textit{Gaussian Process (GP)} is a stochastic process, i.e., a collection of random variables indexed by some input variable, in our case $\theta\in\Theta$, such that every finite linear combination of them is normally distributed.

In practice, a GP defines a distribution over real-valued functions of the form $g: \Theta\rightarrow\mathbb{R}$ and such distribution is uniquely identified by its mean and covariance functions, respectively denoted by $\mu(\theta)=\mathbb{E}[g(\theta)]$ and $k_\gamma(\theta,\theta')$. The GP can thus be denoted as $\mathcal{GP}(\mu(\theta),k_\gamma(\theta,\theta'))$. This means that the function value at any point $\theta$, $g(\theta)$, is a {Gaussian} random variable with mean $\mu(\theta)$ {and variance $k_\gamma(\theta,\theta)$}. The covariance function $k_\gamma(\cdot, \cdot)$ depends on some hyper-parameter $\gamma$. 
Given an input $\theta_i$, let $g_i = g(\theta_i)$ denote its latent variable, i.e., the latent function $g$ evaluated at $\theta_i$. Also denote $g_t = [ g(\theta_i) \mid \theta_i \in \Theta_t ]$, where $\Theta_t$ is the set of input points of the training set $D_t$.  
From $\Theta_t$ it is possible to compute the mean vector $\mu_t$ of the GP, by evaluating the mean function $\mu(\cdot)$ at every point in the set: $\mu_t = [\mu(\theta_i) | \theta_i\in \Theta_t]$. For simplicity and without loss of generality, one can translate the outputs of the training set so to have zero mean, i.e. $\mu_t = \underbar{0}$. Similarly, we define the covariance matrix $K_{N_tN_t}$, by evaluating the covariance function $k_\gamma$ on every pair of points in the set:  $K_{N_tN_t}=[ k_{\gamma}(\theta_i,\theta_j)|\theta_i,\theta_j\in \Theta_t]$. 

GPs model the posterior probabilities by defining latent functions $g:\Theta\to \mathbb{R}$, whose output values are then mapped into the $[0, 1]$ interval
by means of a so-called link function $\Phi$, typically the logit or the probit function, so that $f = g \circ \Phi$.

The first step of a GP algorithm is to place a GP prior over the latent function $g$, defined by 
$$p(g|\Theta_t) = \mathcal{N}(g\mid\underbar{0}, K_{N_tN_t}).$$
Let now consider a test input $\theta_*$ with latent variable $g_*$. In order to do inference, that is, predict the satisfaction function $f_*$, we have to compute 
\begin{equation}\label{eq:pred_gp}
    p(f_*|\theta_*,\Theta_t,L_t) = \int \Phi (g_*)p(g_*|\theta_*, \Theta_t,L_t)dg_*,
\end{equation}
where $L_t$, denotes the set of Boolean tuples corresponding to points in $\Theta_t$.
To compute equation~\eqref{eq:pred_gp}, we have to marginalize the posterior over the latent Gaussian variables:
\begin{equation}\label{eq:post_gp}
    p(g_*|\theta_*, \Theta_t,L_t) = \int p({g}_*|\theta_*, \Theta_t,g_t)p(g_t|\Theta_t,L_t)d g_t,
\end{equation}
where the posterior $p(g_t|\Theta_t,L_t)$ can be obtained using the standard Bayes rule
\[
p(g_t|\Theta_t,L_t)=\frac{p(L_t|g_t,\Theta_t)p(g_t|\Theta_t)}{p(L_t|\Theta_t)}.\]
Therefore, performing inference reduces to solving two integrals, Eq.~\eqref{eq:pred_gp} and \eqref{eq:post_gp}. The second integral is not available in closed form since it is the convolution of a Gaussian distribution, $p(g_t|\Theta_t)$, and a non-Gaussian one, $p(L_t|g_t,\Theta_t)$ which is a binomial distribution. Hence, we have to rely on approximations in order to compute and integrate over the posterior $p(g_t|D_t)$. Once we obtain a tractable approximation of $p(g_*|\theta_*, \Theta_t,L_t)$, we can easily compute an empirical approximation of $p(f_*|\theta_*,\Theta_t,L_t)$.

\subsubsection{Stochastic Variational Inference.}
Here we provide an understanding of how SVI works over GP with non-Gaussian likelihoods. For a more detailed description, we refer the interested reader to~\cite{hensman2013gaussian,hensman2015scalable}. 
Variational approaches to GP start by defining a set of $m$ inducing points $Z = \{z_1,\dots,z_m\}$ that lives in the same space of $\Theta_t$ and, from them, we define a set of inducing variables $u_t = [g(z_i)|z_i\in Z]$. Using standard GP methodologies, one can express:
\begin{align*}
    p(L_t|g_t) &= \prod_{i=1}^{N_t}Binomial(L_i|M_t,\Phi(g_i)),\\
    p(g_t|u_t) &= \mathcal{N}(g_t|K_{N_tm}K_{mm}^{-1}u_t, K_{N_tN_t}-K_{N_tm}K_{mm}^{-1}K_{mN_t}),\\
    p(u_t) &= \mathcal{N}(u_t|\underbar{0},K_{mm}),\\
\end{align*}
where $K_{mm}$ is the covariance function evaluated at the inducing points, $K_{N_t m}$ is the covariance function evaluated between all the inducing and training points and $L_i\in L_t$ is the output associated with input $\theta_i\in\Theta_t$.
Because of Jensen inequality, the log marginal likelihood can be bound as 
\begin{equation}\label{eq:gp_marg_bound}
    \log p(L_t|u_t) \ge \mathbb{E}_{p(g_t|u_t)}[\log p(L_t| g_t)].
\end{equation}
The integral above is in general intractable for the non-conjugate
case.
By substituting~\eqref{eq:gp_marg_bound} in the following standard variational relation
\begin{equation}\label{eq:gp_var}
    \log p(L_t)\ge \mathbb{E}_{q(u_t)}[\log p(L_t|u_t)]-KL[q(u_t)||p(u_t)],
\end{equation}
we obtain the following bound
\begin{equation}\label{eq:gp_bound}
    \log p(L_t)\ge \mathbb{E}_{q(g_t)}[\log p(L_t|g_t)]-KL[q(u_t)||p(u_t)],
\end{equation}
where $q(g_t) = \int p(g_t|u_t)q(u_t)du_t$.
We choose $q(u_t) := \mathcal{N}(u_t|m, \tilde{S})$, where $\tilde{S}$, in order to maintain positive-definiteness, is defined using a lower triangular form, $\tilde{S} := SS^T$. Then
\begin{equation}\label{eq:gp_qg}
    q(g_t) = \mathcal{N}(g_t|Am, K_{N_tN_t}+A(\tilde{S}-K_{mm})A^T,
\end{equation}
where $A = K_{N_tN_t}K_{mm}^{-1}$. Since our
likelihood factors as $p(L_t | g_t ) = \prod_{i=1}^{N_t} p(L_i | g_i )$, the expectation in~\eqref{eq:gp_bound} is the sum of one-dimensional integrals of the log-likelihoods, which can be computed by simple quadrature techniques, and the lower bound becomes:
\begin{equation}\label{eq:gp_svi_bound}
   \log p(L_t)\ge \sum_{i=1}^{N_t}\mathbb{E}_{q(g_i)}[\log p(L_i|g_i)]-KL[q(u_t)||p(u_t)]:= \mathcal{L}_{GP}(m, S, Z, \gamma).
\end{equation}
The SVI algorithm then consists of maximizing $\mathcal{L}_{GP}$, the bound on the
marginal likelihood, with respect to its parameters using  gradient based stochastic optimization. Computing the KL divergence in~\eqref{eq:gp_svi_bound} requires $\mathcal{O}(m^3)$ computations, since the number of inducing points, selected at design time by the user, is much smaller than the number
of data $N_t$, most of the work will be in computing the
expected likelihood terms. In order to compute the gradient of $\mathcal{L}_{GP}$, $\displaystyle \nabla \mathcal{L}_{GP} = [\frac{\partial\mathcal{L}_{GP}}{\partial m}, \frac{\partial\mathcal{L}_{GP}}{\partial S},\frac{\partial\mathcal{L}_{GP}}{\partial Z},\frac{\partial\mathcal{L}_{GP}}{\partial\gamma}]$, we leverage the following identities~\cite{opper2009variational}, where $h$ denotes $\log p(L_i|g_i)$ and $\mu$ and $\sigma^2$ denotes the terms defined in~\eqref{eq:gp_qg} for $q(g_t)$:
\begin{align*}
    \frac{\partial}{\partial\mu}\mathbb{E}_{\mathcal{N}(x|\mu,\sigma^2)}[h(x)] &= \mathbb{E}_{\mathcal{N}(x|\mu,\sigma^2)}\left[\frac{\partial}{\partial x}h(x)\right]\\
    \frac{\partial}{\partial\sigma^2}\mathbb{E}_{\mathcal{N}(x|\mu,\sigma^2)}[h(x)] &= \frac{1}{2} \mathbb{E}_{\mathcal{N}(x|\mu,\sigma^2)}\left[\frac{\partial^2}{\partial x^2}h(x)\right].
\end{align*}
Given the ease of parallelizing
the simple sum over $N_t$, we can optimize $\mathcal{L}_{GP}$ in
a distributed or in a stochastic fashion by selecting mini-batches of the data at random.

\subsubsection{Empirical approximation of the predictive distribution.}
We now approximate the posterior of \eqref{eq:post_gp} as $p(g_*|L_t)\approx \int p(g_*|u_t)q(u_t)du_t: = q(g_*)$. The integral above can be treated similarly to~\eqref{eq:gp_qg}, computing its mean and variance takes $\mathcal{O}(m^2)$. As we can sample from $q(g_*)$, for each input $\theta_*$, we consider $\it [g_*^1,\dots, g_*^C]$ a vector of $C$ samples of $q(g_*)$ and use the link function $\Phi$ to map each $g_*^i$ to the interval $[0,1]$, obtaining a vector $[f_*^1,\dots, f_*^C]$ that empirically approximates $p(f_*|\theta_*, D_t)$ of Eq.~\eqref{eq:pred_gp}. 
By the strong law of large numbers, the empirical approximation converges to the true distribution as $C\to \infty$~\cite{van2000asymptotic}. The sample size $C$ can be chosen, for instance, to ensure a given width of the confidence interval for a statistic of interest~\cite{rasch2011optimal} or to bound the probability that the empirical distribution differs from the true one by at most some given constant~\cite{massart1990tight}.

\subsection{Bayesian Neural Networks}\label{subsec:bnn-smc}

The core idea of Bayesian neural networks (BNNs) is to place a
probability distribution over the weights $\mathbf{w}$ of a neural network $f_{\mathbf{w}}:\Theta\to[0,1]$, transforming the latter into a probabilistic model.

The Bayesian learning process starts by defining a prior distribution for $\mathbf{w}$ that expresses our initial belief about the parameter values. A common choice is to choose a zero-mean Gaussian prior. As we observe data $D_t$, we update this prior to a posterior distribution using Bayes' rule:
\begin{equation}\label{eq:bnn_post}
    p(\mathbf{w}\mid D_t) = \frac{p(D_t\mid \mathbf{w})p(\mathbf{w})}{p(D_t)}.
\end{equation}
Because of the non-linearity introduced by the
neural network function $f_{\mathbf{w}}(\theta)$ and since the likelihood is binomial, the posterior $p(\mathbf{w}|D_t)$ is non-Gaussian and it cannot be computed analytically. 
In order to predict the satisfaction function over an unobserved input $\theta_*$, we marginalize
the predictions with respect to the posterior distribution
of the parameters, obtaining 
\begin{equation}\label{eq:bnn_predictive}
    p(f_*|\theta_*, D_t) = \int f_\mathbf{w}(\theta_*) p(\mathbf{w}|D_t)d\mathbf{w}.
\end{equation}
The latter is called \emph{posterior predictive} distribution and it can be used to retrieve information about the uncertainty of a specific prediction $f_*$.
Unfortunately, the integration is analytically intractable due to the non-linearity of the neural network function~\cite{bishop2006pattern,mackay1992practical}.


\subsubsection{Stochastic Variational Inference.}
%As exact inference is infeasible either with GP and with BNN, we leverage a powerful tool for approximate posterior inference method, Variational Inference (VI)~\cite{jordan1999introduction}.
Given the unknown posterior distribution $p(\mathbf{w}|D_t)$, the rationale of SVI is to choose a family of parametric distributions $q_\psi(\mathbf{w})$, over the same latent variables and minimize the KL divergence between these two distributions, $KL[q_\psi(\mathbf{w})||p(\mathbf{w}|D_t)]$. The goal is to find the members of the family that are closest to the true posterior $p(\mathbf{w}|D_t)$. Since the posterior distribution is not known, a different objective function,
called Evidence Lower Bound (ELBO)~\cite{deodato2019bayesian}, is introduced. In practice, minimizing the KL diverge is equivalent to maximizing the Evidence Lower Bound (ELBO), defined as
\begin{equation}\label{eq:elbo}
    \mathcal{L}_{BNN}(\psi) = \mathbb{E}_{q_\psi(\mathbf{w}|D_t)}\left[\log (D_t|\mathbf{w})\right]-KL\left[q_\psi(\mathbf{w})||p(\mathbf{w})\right].
\end{equation}
The first term is the expected log-likelihood of our data with respect to values of $f_\mathbf{w}$ sampled from $q_\psi(\mathbf{w}|D_t)$, whereas the second term is the KL diverge between the proposal distribution and the prior. The family of distribution $q_\psi$ should be a distribution easy to sample from and such that the KL divergence is easy to compute. A common choice for $q_\psi$ is the Gaussian distribution (where $\psi$ denotes its mean and variance). The KL distribution among two Gaussian distributions has an exact analytical form. Thus, the ELBO of Eq.~\eqref{eq:elbo} can be computed and it can be used as the objective function of a maximization problem over $\psi$.

The predictive distribution~\eqref{eq:bnn_predictive} is a non-linear combination of Gaussian distributions, and thus it is not Gaussian. However, samples can be easily extracted from $q(\mathbf{w}; \psi)$, which allows us to obtain an empirical approximation of the predictive distribution.

\subsubsection{Empirical approximation of the predictive distribution.}
As we can sample from the approximate posterior distribution, we consider $\it [w_1,\dots, w_C]$ denote a vector of $C$ realizations of the random variable $\mathbf{w}\sim q_\psi(\mathbf{w})$. Each realization $w_i$ induces a deterministic function $f_{w_i}$ that can be evaluated at $\theta_*$, the unobserved input, providing an empirical approximation of $p(f_*|\theta_*, D_t)$. 
By the strong law of large numbers, the empirical approximation converges to the true distribution as $C\to \infty$~\cite{van2000asymptotic}. The sample size $C$ can be chosen, for instance, to ensure a given width of the confidence interval for a statistic of interest~\cite{rasch2011optimal} or to bound the probability that the empirical distribution differs from the true one by at most some given constant~\cite{massart1990tight}.
 

==> tables/dataset_training_details.tex <==

%\begin{wraptable}{r}{8cm}
\begin{table}[ht]
\centering
\begin{tabular}{l | c c c c | c c c}
    \toprule
    
    \textbf{Configuration} & \multicolumn{4}{c}{\textbf{Dataset Size}}  & \multicolumn{3}{c}{\textbf{Training time}}\\
     & $N_t$ & $M_t$ & $N_v$ & $M_v$ & EP-GP & SVI-GP & SVI-BNN \\
    \midrule
    $(a)$ SIR $\beta$ & $500$ & $50$ & $1k$ & $1k$& $01.06$ & $\underline{01.11}$ & $03.50$\\
    $(b)$ SIR $\gamma$ & $700$ & $50$ & $1k$ & $1k$ & $02.36$ & $\underline{01.44}$ & $05.24$\\
    $(c)$ SIR $\beta,\gamma$ & $2500$ & $50$ & $400$ & $1k$ & $12.22$ & $\underline{08.12}$ & $19.15$ \\
    \midrule
    $(d)$ PrGeEx $k_2$ & $500$ & $50$ & $400$ & $1k$& $01.39$ & $\underline{01.13}$ & $03.51$\\
    %PrGeEx $k_7$ & $500$ & $50$ & $400$ & $1k$\\
    $(e)$ PrGeEx $k_2, k_7$ & $2500$ & $50$ & $400$ & $1k$ & $22.11$ & $\underline{08.31}$ & $19.10$\\
    \midrule
    $(f)$ PhosRelay $k_1$ & $500$ & $50$ & $1k$ & $1k$ & $01.00$ & $\underline{01.20}$ & $03.51$\\
    $(g)$ PhosRelay $k_p,k_d$ & $2500$ & $50$ & $400$ & $1k$& $06.57$ & $\underline{08.70}$ & $19.39$ \\
    $(h)$ PhosRelay $k_1,k_2,k_3$ & $8k$ & $20$ & $1k$ & $1k$ & $36.13$ & $\underline{26.38}$ & $66.30$\\
    $(i)$ PhosRelay $k_1,\ldots,k_4$ & $10k$ & $20$ & $4096$ & $1k$ & $45.59$ & $\underline{33.45}$ & $81.16$\\
    $(l)$ PhosRelay $k_p,k_1,\ldots,k_4,k_d$ & $1000k$ & $20$ & $4096$ & $1k$& $-$ & $\underline{286.33}$ & $\underline{92.30}$\\
    Random pCTMC & $5k\cdot r$ & $10$ & $100\cdot r$ & $1k$ &  &  & \\
    \bottomrule
\end{tabular}
\caption{Size of training ($D_t$) and test ($D_v$) datasets and training time (min) for EP-GP, SVI-GP and SVI-BNN. $N_t$ and $N_v$ denote the number of parameter values, while $M_t$ and $M_v$ denote the number of Bernoulli observations for each parameter value. Underlined values correspond to GPU computations. EP-GP training time for the last configuration is not reported due to memory timeout. \vspace{-0.5cm}}
\label{tab:dataset_size_time}
\end{table}
%\end{wraptable}

==> tables/eval_times.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{p{4cm}|c c}
    \toprule
    \textbf{Dataset} & \multicolumn{2}{c}{\textbf{Evaluation time} (min)} \\
    & SVI-GP & SVI-BNN \\
    \midrule
    SIR $\beta$ & $00.36$ & $00.10$\\
    SIR $\gamma$ & $00.48$ & $00.10$ \\
    SIR $\beta,\gamma$ & $00.18$ & $00.00$ \\
    \midrule
    PrGeEx $k_2$ & $00.17$ & $00.10$ \\
    PrGeEx $k_7$ & \\
    PrGeEx $k_2, k_7$ & $00.14$ & $00.00$ \\
    \midrule
    PhosRelay $k_1$ & $00.25$ & $00.10$\\
    PhosRelay $k_p,k_d$ & $00.10$ & $00.20$\\
    PhosRelay $k_1,k_2,k_3$ & $01.10$ & $00.26$\\
    PhosRelay $k_1,\ldots,k4$ & $04.11$ & $01.60$\\
    PhosRelay $k_p,k_1,\ldots,k_4,k_d$ & & $00.13$\\
    \bottomrule
\end{tabular}
\caption{Evaluation time (min) on CPU for SVI-GP and SVI-BNN models with $1k$ posterior samples on the datasets presented in Section \ref{sec:case_studies}.}
\label{tab:eval_time}
\end{table}


==> tables/perf_metrics.tex <==
\begin{table}[ht]
\centering
\adjustbox{max width=\textwidth, max height=\textheight}{
\begin{tabular}{l|c c c | c c c}
    \toprule
    \textbf{Configuration} & \multicolumn{3}{c}{\textbf{MSE}} & \multicolumn{3}{c}{\textbf{Test accuracy}} \\
    & EP-GP & SVI-GP & SVI-BNN &  EP-GP & SVI-GP & SVI-BNN \\
    \hline
    $(a)$ SIR $\beta$ & $1.99$ & $\mathbf{1.90}$ & $2.05$ & $\mathbf{100.00}$ & $98.80$ & $\mathbf{100.00}$\\
    $(b)$ SIR $\gamma$ & $1.05$ & $\mathbf{0.71}$ & $0.93$& $77.80$ & $77.30$ & $\mathbf{92.60}$\\
    $(c)$ SIR $\beta,\gamma$ & $1.57$ & $1.45$ &$\mathbf{0.98}$& $72.75$ & $85.75$ & $\mathbf{92.25}$ \\
    \hline
    $(d)$ PGE $k_2$ & $\mathbf{28.52}$ & $33.95$ & $30.39$ & $93.75$ & $94.00$ & $\mathbf{97.50}$\\
    $(e)$ PGE $k_2, k_7$ & $41.96$ & $11.85$ & $\mathbf{4.24}$ & $78.25$ & $89.25$ & $\mathbf{95.00}$\\
    \hline
    $(f)$ PR $k_1$ & $5.06$ & $3.96$ & $\mathbf{3.17}$& $99.70$ & $99.20$ & $\mathbf{100.00}$\\
    $(g)$ PR $k_p,k_d$ & $8.68$ & $5.32$ & $\mathbf{3.59}$ & $99.25$ & $96.25$ & $\mathbf{99.75}$\\
    $(h)$ PR $k_1,k_2,k_3$ & $48.66$ & $5.28$ & $\mathbf{4.05}$  & $99.80$ & $93.70$ & $\mathbf{100.0}$  \\
    $(i)$ PR $k_1,\ldots,k_4$ &  $113.11$ & $\mathbf{5.97}$ & $7.11$& $99.02$ & $93.65$ & $\mathbf{99.92}$\\
    $(l)$ PR $k_p,k_1,\ldots,k_4,k_d$ & 
    - & $3.50$ & $\mathbf{2.43}$  & - & $97.02$ & $\mathbf{99.80}$ \\
    
    \bottomrule
\end{tabular}}
\caption{Mean Squared Error ($\times10^{-4}$) and test accuracy ($\%$) for EP-GP, SVI-GP and SVI-BNN. SVI-BNNs are evaluated on $1k$ posterior samples. For each case study, we highlight the minimum MSE and the highest accuracy values. \vspace{-1cm}}
\label{tab:mse_acc}
\end{table}



\begin{table}[ht]
\centering
\begin{tabular}{l|c c c c}
    \toprule
    \textbf{Configuration} & \textbf{Test set} & \textbf{EP-GP} & \textbf{SVI-GP} & \textbf{SVI-BNN} \\
    \hline
    $(a)$ SIR $\beta$ & $0.044$ & $0.044$ & $\color{Blue}\underline{ 0.032}$ & $\color{Red}\overline{ 0.097}$ \\
    $(b)$ SIR $\gamma$ & $0.018$ & $0.018$ & $\color{Blue}\underline{ 0.012}$ & $\color{Red}\overline{0.058}$\\
    $(c)$ SIR $\beta,\gamma$ & $\color{Blue}\underline{0.019}$ & $0.042$ & $\color{Blue}\underline{0.019}$ & $\color{Red}\overline{0.047}$\\
    \hline
    $(d)$ PGE $k_2$ & $0.039$ & $\color{Blue}\underline{0.030}$ & $0.037$ & $\color{Red}\overline{0.080}$\\
    $(e)$ PGE $k_2, k_7$ & $0.043$ & $\color{Blue}\underline{0.021}$ & $0.056$ & $\color{Red}\overline{0.093}$ \\
    \hline
    $(f)$ PR $k_1$ & $0.058$ & $0.059$ & $\color{Blue}\underline{0.046}$ & $\color{Red}\overline{0.100}$\\
    $(g)$ PR $k_p,k_d$ & $0.055$ & $\color{Red}\overline{0.108}$ & $\color{Blue}\underline{0.037}$ & $0.093$\\
    $(h)$ PR $k_1,k_2,k_3$ & $0.050$ & $\color{Red}\overline{0.340}$ & $\color{Blue}\underline{0.030}$ & $0.121$\\
    $(i)$ PR $k_1,\ldots,k_4$ & $0.050$ & $\color{Red}\overline{0.682}$ & $\color{Blue}\underline{0.030}$ & $0.150$\\
    $(l)$ PR $k_p,k_1,\ldots,k_4,k_d$ & $0.049$ & - & $\color{Blue}\underline{0.028}$ & $\color{Red}\overline{0.087}$\\
    \bottomrule
\end{tabular}
\caption{Average uncertainty width for EP-GP, SVI-GP and SVI-BNN compared to the average uncertainty width of the test set. SVI-BNNs are evaluated on $1k$ posterior samples. For each case study we highlight the \textcolor{Blue}{lowest} and \textcolor{Red}{highest} uncertainty values.\vspace{-1cm}}
\label{tab:unc_area}
\end{table}

==> tables/training_times.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{p{4cm}|c c c }
    \toprule
    \textbf{Dataset} & \multicolumn{3}{c}{\textbf{Training time} (min)} \\
    & EP-GP & SVI-GP & SVI-BNN \\
    \midrule
    SIR $\beta$ & $01.06$ & $\underline{01.11}$ & $03.50$\\
    SIR $\gamma$ & $02.36$ & $\underline{01.44}$ & $05.24$\\
    SIR $\beta,\gamma$ & $12.22$ & $\underline{08.12}$ & $19.15$ \\
    \midrule
    PrGeEx $k_2$ & $01.39$ & $\underline{01.13}$ & $03.51$\\
    PrGeEx $k_7$ & & & \\
    PrGeEx $k_2, k_7$ & $22.11$ & $\underline{08.31}$ & $19.10$\\
    \midrule
    PhosRelay $k_1$ & $01.00$ & $\underline{01.20}$ & $03.51$\\
    PhosRelay $k_p,k_d$ & $06.57$ & $\underline{08.70}$ & $19.39$ \\
    PhosRelay $k_1,k_2,k_3$ & $36.13$ & $\underline{26.38}$ & $66.30$\\
    PhosRelay $k_1,\ldots,k4$ & $45.59$ & $\underline{33.45}$ & $81.16$\\
    PhosRelay $k_p,k_1,\ldots,k_4,k_d$ & $-$ &  & \\
    \bottomrule
\end{tabular}
\caption{Training time (min) for EP-GP, SVI-GP and SVI-BNN models on the datasets presented in Section~\ref{sec:case_studies}. Underlined values correspond to GPU computations.}
\label{tab:train_time}
\end{table}


% OLD TABLE % 

% \begin{table}[ht]
% \centering
% \begin{tabular}{p{4cm}|c c c c c}
%     \toprule
%     \textbf{Dataset} & \multicolumn{3}{c}{\textbf{CPU training time} (min)} & \multicolumn{2}{c}{\textbf{CPU evaluation time} (min)} \\
%     & EP GP & SVI GP & SVI BNN & SVI GP & SVI BNN\\
%     \midrule
%     SIR $\beta$ & $30.24$ & $67.14$ & $07.53$ & $00.36$ & $00.10$\\
%     SIR $\gamma$ & $45.35$ & $65.22$ & $07.56$ & $00.48$ & $00.10$ \\
%     SIR $\beta,\gamma$ & $102.23$ & $577.43$ & $39.43$ & $00.18$ & $00.00$ \\
%     \midrule
%     PrGeEx $k_2$ & $24.47$ & $76.42$ & $08.00$ & $00.17$ & $00.10$ \\
%     PrGeEx $k_7$ & \\
%     PrGeEx $k_2, k_7$ & $111.25$ & $247.25$ & $39.52$ & $00.14$ & $00.00$ \\
%     \midrule
%     PhosRelay $k_1$ & $24.20$ & $32.57$ & $09.21$ & $00.25$ & $00.10$\\
%     PhosRelay $k_p,k_d$ & $47.40$ & $600.03$ & $39.40$ & $00.10$ & $00.20$\\
%     PhosRelay $k_1,k_2,k_3$ & $114.28$ & $618.12$ & $128.3$ & $01.10$ & $00.40$\\
%     PhosRelay $k_1,\ldots,k4$ & $119.56$ & $126.40$ & $161.23$ & $04.11$ & $00.12$\\
%     PhosRelay $k_p,k_1,\ldots,k_4,k_d$ & - & \\
%     \bottomrule
% \end{tabular}
% \caption{CPU training time for EP-GP, SVI-GP and SVI-BNN models and evaluation time with $1k$ posterior samples for SVI-GPs and SVI-BNNs on the datasets presented in Section \ref{sec:case_studies}.}
% \label{tab:time}
% \end{table}


